Hide and Speak: Towards Deep Neural Networks for Speech Steganography

Steganography is the science of hiding a secret message within an ordinary public message, which is referred to as Carrier. Traditionally, digital signal processing techniques, such as least significant bit encoding, were used for hiding messages. In this paper, we explore the use of deep neural networks as steganographic functions for speech data. We showed that steganography models proposed for vision are less suitable for speech, and propose a new model that includes the short-time Fourier transform and inverse-short-time Fourier transform as differentiable layers within the network, thus imposing a vital constraint on the network outputs. We empirically demonstrated the effectiveness of the proposed method comparing to deep learning based on several speech datasets and analyzed the results quantitatively and qualitatively. Moreover, we showed that the proposed approach could be applied to conceal multiple messages in a single carrier using multiple decoders or a single conditional decoder. Lastly, we evaluated our model under different channel distortions. Qualitative experiments suggest that modifications to the carrier are unnoticeable by human listeners and that the decoded messages are highly intelligible.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}
In standard steganographic applications it is assumed that the original, clean, carrier is kept private and can not be accessed by an adversary. However, in order to further analyze the ability of the generated carrier to encode the hidden message, we experienced with subtracting the original carrier from the embedded carrier and visualizing the resulted spectrograms. 

Carrier visualizations consist of the original unmodified carrier, the carrier embedded with a hidden message and their residual difference. Message visualizations consist of the original message, the message decoded by the steganograpy model and their residual difference. We notice that the residual difference, both in audio form and visual representation, is not sufficient evidence to decypher the embedded message.

In some cases, $(\hat{\cf}-\cf)$ vaguely resembles $\m$ in the ears of a human listener when presented with the original message~\cite{spieth1954responding}. Such setup where the adversary has access to the original carrier and some reference of the original message is extreme and highly unlikely. 

Nevertheless, additional precautions can be taken to further obfuscate the hidden message and challenge such adversary. One can utilize many pre-processing stages before passing it to the steganography function, such as: frequency permutation, dividing the spectrograms to tiles and re-arranging, etc. In this study we explore a more basic operation of time and frequency flipping of the message. We flip the message spectrogram along the time and frequency axes and feed it to the steganography model. We leave additional and more intricate transformations for future work.

The above pre-processing stage results in a incomprehensible $(\hat{\cf}-\cf)$ while retaining the same message reconstruction ability after repeating the flipping operation. 

Figure~\ref{fig:specdiff} presents visualizations of carrier and message for a single message decoding, preprocessed single message decoding and three messages decoding. Notice, in single message decoding the residual difference resembles the embedded message in areas of high energy, both visually and audibly. When preprocessing the message, although the residual difference resembles the message visually, it is incomprehensible to a human listener. This visual similarity can be mitigated using more complex transformations as described above. Lastly, in multiple messages decoding, the residual difference appears to be very noisy and bares no resemblance to any particular single embedded message.

\begin{figure*}[t]
\centering
% regular
\includegraphics[width=0.49\linewidth]{figures/cerdiff_1.pdf}
\includegraphics[width=0.49\linewidth]{figures/msgdiff_1.pdf}\\
% \includegraphics[width=0.49\linewidth]{figures/cerdiff_2.pdf}
% \includegraphics[width=0.49\linewidth]{figures/msgdiff_2.pdf}
% \\

% flipped
\includegraphics[width=0.49\linewidth]{figures/cerdiff_flip_2.pdf}
\includegraphics[width=0.49\linewidth]{figures/msgdiff_flip_2.pdf}\\

% 3 msg
\includegraphics[width=0.49\linewidth]{figures/cerdiff_3.pdf}
\includegraphics[width=0.49\linewidth]{figures/msgdiff_3.pdf}

% flipped
% \includegraphics[width=0.49\linewidth]{figures/cerdiff_flip.pdf}
% \includegraphics[width=0.49\linewidth]{figures/msgdiff_flip.pdf}
% \\
% \includegraphics[width=0.49\linewidth]{figures/cerdiff_flip_1.pdf}
% \includegraphics[width=0.49\linewidth]{figures/msgdiff_flip_1.pdf}
% \\
\caption{Steganography results. 
First three images of each set: original carrier $\cf$, embedded carrier $\hat{\cf}$ and their residual error. Last three images of each set: original message $\m$, decoded message $\hat{\m}$ and their residual error. The first row corresponds to a single message decoding, the second row corresponds to decoding a single preprocessed message, and the last row corresponds to decoding three messages using three decoders.}
\label{fig:specdiff}
\end{figure*}
